FAMA: Failure-Aware Meta-Agentic Framework for Open-Source LLMs in Interactive Tool Use Environments

Large Language Models are being increasingly deployed as the decision-making core of autonomous agents capable of effecting change in external environments. Yet, in conversational benchmarks, which simulate real-world customer-centric issue resolution scenarios, these agents frequently fail due to the cascading effects of incorrect decision-making. These challenges are particularly pronounced for open-source LLMs with smaller parameter sizes, limited context windows, and constrained inference budgets, which contribute to increased error accumulation in agentic settings. To tackle these challenges, we present the Failure-Aware Meta-Agentic (FAMA) framework. FAMA operates in two stages: first, it analyzes failure trajectories from baseline agents to identify the most prevalent errors; second, it employs an orchestration mechanism that activates a minimal subset of specialized agents tailored to address these failures by injecting a targeted context for the tool-use agent before the decision-making step. Experiments across open-source LLMs demonstrate performance gains up to 27% across evaluation modes over standard baselines. These results highlight that targeted curation of context through specialized agents to address common failures is a valuable design principle for building reliable, multi-turn tool-use LLM agents that simulate real-world conversational scenarios.

==> tables/main_results_tau_bench_tau_trait_pass_hat_1_5.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lrrrrrrrr}
\toprule
\textbf{Method} 
& \multicolumn{2}{c}{$\tau$-Airline} 
& \multicolumn{2}{c}{$\tau$-Retail} 
& \multicolumn{2}{c}{$\tau$-Telehealth} 
& \multicolumn{2}{c}{$\tau$-Telecom} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
& P@1 & P@5 & P@1 & P@5 & P@1 & P@5 & P@1 & P@5 \\
\midrule

\multicolumn{9}{l}{\textbf{\textit{Qwen3-4B-Instruct}}} \\
\addlinespace[3pt]
ReAct & \underline{32.00} & \underline{26.00} & 17.22 & 8.70 & 22.99 & 10.00 & 15.55 & 5.55 \\
FC    & 27.60 & 14.00 & 24.90 & 9.00 & \textbf{34.00} & \textbf{20.00} & 37.00 & 21.00 \\
IRMA  & 30.00 & 12.00 & \underline{28.86} & \underline{9.56} & 22.99 & 10.00 & 38.00 & 16.00 \\
FAMA (\textbf{our}) 
      & \textbf{37.60} & \textbf{26.00} & \textbf{34.60} & \textbf{13.90} 
      & 32.00 & 17.00 & \textbf{39.00} & \textbf{17.00} \\
\addlinespace[3pt]
\hdashline

\addlinespace[3pt]
\multicolumn{9}{l}{\textit{\textbf{Qwen3-14B}}} \\
\addlinespace[3pt]
ReAct & 18.40 & 8.00 & 25.20 & 12.10 & \textbf{44.00} & \textbf{40.00} & 15.55 & 11.11 \\
FC    & 14.00 & 8.00 & \underline{32.60} & \underline{13.00} & 39.00 & 35.00 & 38.00 & 27.00 \\
IRMA  & \underline{36.40} & \textbf{18.00} & 28.50 & 6.90 & 39.99 & 20.00 & 36.66 & 11.11 \\
FAMA (\textbf{our}) 
      & \textbf{36.80} & \underline{16.00} & \textbf{37.90} & \textbf{14.70} 
      & 42.00 & 40.00 & \textbf{43.00} & \textbf{28.00} \\
\addlinespace[3pt]
\hdashline

\addlinespace[3pt]
\multicolumn{9}{l}{\textit{\textbf{Qwen3-32B}}} \\
\addlinespace[3pt]
ReAct & \textbf{30.40} & \underline{14.00} & \underline{38.00} & 10.00 & \underline{43.00} & 30.00 & 24.44 & 16.66 \\
FC    & 17.60 & 10.00 & 35.00 & \underline{11.00} & 42.00 & \underline{35.00} & 32.00 & 16.00 \\
IRMA  & 24.40 & 8.00 & 26.90 & 6.90 & 30.00 & 15.00 & \underline{40.00} & 22.20 \\
FAMA (\textbf{our}) 
      & \underline{26.80} & \textbf{18.00} & \textbf{40.50} & \textbf{12.20} 
      & \textbf{45.00} & \textbf{35.00} & \textbf{37.77} & \textbf{27.77} \\
\addlinespace[3pt]
\hdashline

\addlinespace[3pt]
\multicolumn{9}{l}{\textit{\textbf{Qwen2.5-72B-Instruct}}} \\
\addlinespace[3pt]
ReAct & 24.40 & \underline{10.00} & \underline{43.47} & \underline{20.86} & \underline{43.00} & 22.00 & 51.11 & 22.22 \\
FC    & 15.20 & 2.00 & 19.65 & 4.34 & 41.00 & 30.00 & 44.00 & 27.00 \\
IRMA  & \underline{26.40} & \underline{10.00} & 38.78 & 19.13 & 31.00 & 25.00 & 44.44 & 22.22 \\
FAMA (\textbf{our}) 
      & \textbf{29.20} & \textbf{18.00} & \textbf{44.17} & \textbf{26.95} 
      & \textbf{42.00} & \textbf{40.00} & \textbf{52.00} & \textbf{39.00} \\

\bottomrule
\end{tabular}
\caption{Comparison of different open-source agents on $\tau$-bench across domains using Pass@1 and Pass@5.}
\label{tab:tau_bench_all_pass1_pass5}
\end{table*}
